Learning Probabilistic Models of Word Sense Disambiguation

This dissertation presents several new methods of supervised and unsupervised learning of word sense disambiguation models. The supervised methods focus on performing model searches through a space of probabilistic models, and the unsupervised methods rely on the use of Gibbs Sampling and the Expectation Maximization (EM) algorithm. In both the supervised and unsupervised case, the Naive Bayesian model is found to perform well. An explanation for this success is presented in terms of learning rates and bias-variance decompositions.

==> junk/bv.tex <==

\subsection{Bias Variance Decompositions}
\label{sec:backbv}

A loss function measures the difference between a predicted value for 
a variable and the true value. For classification problems the
zero--one loss function is typically employed. This implies that there
is one correct classification and that all errors are of equal
weight. 

function is simply the percentage of instances in the test set that are 
misclassified. Simply put:
\begin{equation}
classification \ \  error = 1.00 - accuracy
\end{equation}

This is often called {\it zero--one loss} and implies that there is
only one correct classification and that all errors are of equal
weight. 

Mean--squared error is another form of loss function. 
decomposed into bias
and variance components
in \cite{GemanBD92}. This is a useful tool in analyzing the results of
regression problems. However, it is not applicable to classification
where error is measured by counting the number of misclassifications. 

In recent years a number of decompositions of classification error rate
into more fundamental components have been proposed. In general these
decompositions show that:
\begin{equation}
classification \ \  error = bias^2 + variance;
\end{equation}

Bias is an estimate of the systematic error that a learning algorithm
is expected to make.  Variance estimates the degree to which the
learning algorithm is affected by variations in the training
sample. 

The first such decomposition was suggested by \cite{KongD95}. This was
later refined by  \cite{KohaviW96}, \cite{Tibshirani96}, 
\cite{Friedman97}, and \cite{JamesH97}. 

This dissertation follows the decomposition proposed in  \cite{KohaviW96} 
since it adheres to the more generalized loss--function decompositions 
developed in \cite{Tibshirani96} and \cite{JamesH97} and is also 
implemented in the software package MLC++ \cite{KohaviSD96}.   



==> junk/chap6-adj.tex <==

\begin{figure}
\input{figs/chiefa.tex}
\caption{Learning Rate for Adjective {\it chief}}
\label{fig:lrchief}
\vskip -0.14in
\end{figure}

\begin{figure}
\input{figs/commona.tex}
\caption{Learning Rate for Adjective {\it common}}
\label{fig:lrcommon}
\vskip -0.14in
\end{figure}

\begin{figure}
\input{figs/lasta.tex}
\caption{Learning Rate for Adjective {\it last}}
\label{fig:lrlast}
\vskip -0.14in
\end{figure}

\begin{figure}
\input{figs/publica.tex}
\caption{Learning Rate for Adjective {\it public}}
\label{fig:lrpublic}
\vskip -0.14in
\end{figure}






==> junk/chap6-noun.tex <==
\begin{figure}
\input{figs/billa.tex}
\caption{Learning Rate for Noun {\it bill}}
\label{fig:lrbill}
\vskip -0.14in
\end{figure}

\begin{figure}
\input{figs/concerna.tex}
\caption{Learning Rate for Noun {\it concern}}
\label{fig:lrconcern}
\vskip -0.14in
\end{figure}

\begin{figure}
\input{figs/druga.tex}
\caption{Learning Rate for Noun {\it drug}}
\label{fig:lrdrug}
\vskip -0.14in
\end{figure}

\begin{figure}
\input{figs/interesta.tex}
\caption{Learning Rate for Noun {\it interest}}
\label{fig:lrinterest}
\vskip -0.14in
\end{figure}





==> junk/chap6-verb.tex <==
\begin{figure}
\input{figs/agreea.tex}
\caption{Learning Rate for Verb {\it agree}}
\label{fig:lragree}
\vskip -0.14in
\end{figure}

\begin{figure}
\input{figs/closea.tex}
\caption{Learning Rate for Verb {\it close}}
\label{fig:lrclose}
\vskip -0.14in
\end{figure}

\begin{figure}
\input{figs/helpa.tex}
\caption{Learning Rate for Verb {\it help}}
\label{fig:lrhelp}
\vskip -0.14in
\end{figure}

\begin{figure}
\input{figs/includea.tex}
\caption{Learning Rate for Verb {\it include}}
\label{fig:lrinclude}
\vskip -0.14in
\end{figure}




==> junk/em-example.tex <==
\input{head.tex}
\begin{thesis}

\chapter{EM}

The step by step operation of the EM algorithm is illustrated with a
simple example. Suppose that there is a data sample where events are
described by 3 random variables. The variables $F_1$ and $F_2$ are
observed and have two  possible values. The variable $S$ represents
the class of the event but is unobserved. The data sample used in this
example has 10 observations and is shown in Table \ref{tab:data}.   

\begin{table}
\begin{center}
\caption{Unsupervised Learning Example Data}
\label{tab:data}
\begin{tabular}{cc|c} 
$F_1$ & $F_2$ & S \\ \hline
1 & 2 & ?  \\   
1 & 2 & ?  \\
2 & 2 & ?  \\ 
2 & 2 & ?  \\
1 & 2 & ?  \\
1 & 1 & ?  \\
1 & 1 & ?  \\
1 & 1 & ?  \\
1 & 2 & ?  \\
2 & 2 & ?  \\ 
\end{tabular}
\end{center}
\myendtab

It is assumed that Naive Bayes is  the parametric form of the model:  
\begin{equation}
\hat p(F_1,F_2,S) = \hat p(S) \times \hat p(F_1|S) \times \hat p(F_2|S)
\end{equation}

{\bf E--Step Iteration 1}: The EM algorithm begins by randomly
assigning values to $S$. Such an assignment is shown on the left side
of Figure \ref{fig:estep1}. Given these random assignments, estimated
values for the sufficient statistics of the Naive Bayes model are
made. The sufficient statistics are the frequency counts of the
marginal events, i.e., $freq(F_1,S)$ and $freq(F_2,S)$. 
The marginal event counts are conveniently represented in a
cross--classification or contingency table, as shown in the center and
right of Figure \ref{fig:estep1}. The center table shows, for example
that $freq(F_1=1,S=1) = 3$, $freq(F_1=2,S=1) = 1$,  and
$freq(S=1) = 4$. 

\begin{figure}
\begin{center}
\begin{tabular}{cc|ccc}
$F_1$ & $F_2$ & S  & & \\  
\cline{1-3}
1 & 2 & 1 & &  \\
1 & 2 & 3 & &  \\
2 & 2 & 2 & &  \\
2 & 2 & 2 & &  \\
1 & 2 & 1 & &  \\
1 & 1 & 3 & &  \\
1 & 1 & 1 & &  \\
1 & 1 & 2 & &  \\
1 & 2 & 2 & &  \\
2 & 2 & 1 & &  \\ 
\end{tabular}
\begin{tabular}{cc|cc|ccc} 
\multicolumn{2}{c}{} & 
\multicolumn{2}{c}{$F_1$} & 
\multicolumn{3}{c}{} \\
  &   &  1  &  2 & & &   \\ 
\cline{2-5}
  & 1 &  3  &  1 & 4 & &  \\
S & 2 &  2  &  2 & 4 & & \\
  & 3 &  2  &  0 & 2 & & \\
\cline{2-5}
  &   &  7  &  3 & 10 & & \\ 
\end{tabular}
\begin{tabular}{cc|cc|ccc} 
\multicolumn{2}{c}{} & 
\multicolumn{2}{c}{$F_2$} & 
\multicolumn{3}{c}{} \\
  &   &  1  &  2 &  & &   \\ 
\cline{2-5}
  & 1 &  1  &  3 & 4 & &  \\
S & 2 &  1  &  3 & 4 & &  \\
  & 3 &  1  &  1 & 2 & &  \\
\cline{2-5}
  &   &  7  &  3 & 10 & & \\ 
\end{tabular}
\caption{E--Step Iteration 1}
\label{fig:estep1}
\end{center}
\myendfig   

{\bf M---Step Iteration 1:}
Maximum likelihood estimates for the parameters of Naive Bayes are
made from the marginal event counts found during the E--step. Given the
marginal event counts in Figure \ref{fig:estep1}, the parameter estimates 
are computed via:
\begin{eqnarray}
\hat p(S) = \frac{freq(S)}{N} \ \ , \ \ \hat p(F_i|S) =
\frac{freq(F_i,S)}{freq(S)} 
\end{eqnarray}
The values for these estimates are shown in Figure \ref{fig:mstep1}.  

\begin{figure}
\begin{center}
\begin{tabular}{cc|c|ccc} 
  &   &         & & & \\
\cline{2-4}
  & 1 &  0.4    & & &  \\
S & 2 &  0.4    & & & \\
  & 3 &  0.2    & & & \\
\cline{2-4} 
  &   &         & & & \\ 
\end{tabular}
\begin{tabular}{cc|cc|cccc} 
\multicolumn{2}{c}{} & 
\multicolumn{2}{c}{$F_1$} & 
\multicolumn{4}{c}{} \\ 
  &   &  1     &  2    &      & & & \\
\cline{2-5}
  & 1 &  0.75  &  0.25 & 1.0 & & &  \\
S & 2 &  0.50  &  0.50 & 1.0 & & &  \\
  & 3 &  1.00  &  0.00 & 1.0 & & &  \\
\cline{2-5} 
  &   &        &       &      & & &  \\ 
\end{tabular}
\begin{tabular}{cc|cc|cc} 
\multicolumn{2}{c}{} & 
\multicolumn{2}{c}{$F_2$} & 
\multicolumn{2}{c}{} \\ 
  &   &  1     &  2   &   &  \\
\cline{2-5}
  &1  & 0.25  & 0.75 & 1.0 &  \\
S &2  & 0.25  & 0.75 & 1.0 &  \\
  &3  & 0.50  & 0.50 & 1.0 &  \\
\cline{2-5} 
  &   &       &      &     & \\ 
\end{tabular}
\caption{M--step Iteration 1:  $\hat p(S)$ (left), $\hat p(F_1|S)$ (center),
$\hat p(F_2|S)$ (right)} 
\label{fig:mstep1}
\end{center}
\myendfig   

{\bf E--Step Iteration 2:}
After the first iteration of the EM algorithm, all subsequent
iterations re--estimate the marginal event counts by imputing new
values for $S$ from the following equation:
\begin{equation}
S = \stackrel{argmax}{s} \hat p(S | F_1, F_2) = \frac{\hat p(S) \times
\hat p(F_1|S) \times \hat p(F_2|S)}{\hat p(F_1,F_2)} 
\label{eq:finds}
\end{equation}

The estimates of the parameters required by Equation \ref{eq:finds}
are the estimates made in the M--step of the previous iteration, shown 
in Figure \ref{fig:mstep1}. The computation in Equation \ref{eq:finds}
results in the value of $S$ that maximizes a conditional probability
distribution where $S$ is conditioned on the values of the observed
features $F_1$ and $F_2$.  The estimated values of $\hat p(S|F_1,F_2)$
are shown in Figure \ref{fig:estep2}. The maximum probability for each
possible pair of observed features $(f_1, F_2)$ is shown in bold face
and the associated value for $S$ is assigned to all such pairs of
features that occur in the data sample. 

\begin{figure}
\begin{center}
\begin{tabular}{ccc|c}
$F_1$ & $F_2$ & $S$ & $p(S|F_1,F_2)$ \\  \hline
 1    &   1   &  1  &  .333  \\
 1    &   1   &  2  &  .222  \\
 1    &   1   &  3  &  {\bf .444}  \\ \hline
 1    &   2   &  1  &  {\bf .474}  \\
 1    &   2   &  2  &  .316  \\
 1    &   2   &  3  &  .211  \\ \hline
 2    &   1   &  1  &  .333  \\
 2    &   1   &  2  &  {\bf .667}  \\
 2    &   1   &  3  &  .000  \\  \hline
 2    &   2   &  1  &  .333  \\
 2    &   2   &  2  &  {\bf .667}  \\
 2    &   2   &  3  &  .000  \\
\end{tabular}
\caption{E--Step Iteration 2}
\label{fig:estep2}
\end{center}
\myendfig   

\begin{figure}
\begin{center}
\begin{tabular}{cc|ccc}
$F_1$ & $F_2$ & S \\  
\cline{1-3}
1 & 2 & 1 & &  \\
1 & 2 & 1 & &  \\
2 & 2 & 2 & &  \\
2 & 2 & 2 & &  \\
1 & 2 & 1 & &  \\
1 & 1 & 3 & &  \\
1 & 1 & 3 & &  \\
1 & 1 & 3 & &  \\
1 & 2 & 1 & &  \\
2 & 2 & 2 & &  \\ 
\end{tabular}
\begin{tabular}{cc|cc|ccc} 
\multicolumn{2}{c}{} & 
\multicolumn{2}{c}{$F_1$} & 
\multicolumn{3}{c}{} \\
  &   &  1  &  2 &  & &   \\ 
\cline{2-5}
  & 1 &  4  &  0 & 4 & &  \\
S & 2 &  0  &  3 & 3 & &  \\
  & 3 &  3  &  0 & 3 & &  \\
\cline{2-5}
  &   &  7  &  3 & 10 & & \\ 
\end{tabular}
\begin{tabular}{cc|cc|ccc} 
\multicolumn{2}{c}{} & 
\multicolumn{2}{c}{$F_2$} & 
\multicolumn{3}{c}{} \\
  &   &  1  &  2 &  & &   \\ 
\cline{2-5}
  & 1 &  0  &  4 & 4 & &  \\
S & 2 &  0  &  3 & 3 & &  \\
  & 3 &  3  &  0 & 3 & &  \\
\cline{2-5}
  &   &  3  &  7 & 10 & &  \\ 
\end{tabular}
\caption{E--Step Iteration 2}
\label{fig:estep2a}
\end{center}
\myendfig   

The data sample with newly updated values for $S$ is shown on the
left of Figure \ref{fig:estep2a}. The contingency table
representations of this data are shown in the center and on the right
of this same figure and contain the new values of the expected
marginal event counts.   

{\bf M--Step Iteration 2:}
Given the expected values of the  marginal event counts from the
previous E--step, values for the model parameters are re--estimated.
Figure  \ref{fig:mstep2} shows the estimates for $p(S)$, $p(F_1|S)$,
and  $p(F_2|S)$. 

\begin{figure}
\begin{center}
\begin{tabular}{cc|c|ccc} 
  &   &         & & & \\
\cline{2-4}
  & 1 &  0.4    & & &  \\
S & 2 &  0.3    & & & \\
  & 3 &  0.3    & & & \\
\cline{2-4} 
  &   &         & & & \\ 
\end{tabular}
\begin{tabular}{cc|cc|cccc} 
\multicolumn{2}{c}{} & 
\multicolumn{2}{c}{$F_1$} & 
\multicolumn{4}{c}{} \\ 
  &   &  1     &  2    &      & & & \\
\cline{2-5}
  & 1 &  1.0  &  0.0 & 1.0 & & &  \\
S & 2 &  0.0  &  1.0 & 1.0 & & &  \\
  & 3 &  1.0  &  0.0 & 1.0 & & &  \\
\cline{2-5} 
  &   &        &       &   & & &  \\ 
\end{tabular}
\begin{tabular}{cc|cc|cc} 
\multicolumn{2}{c}{} & 
\multicolumn{2}{c}{$F_2$} & 
\multicolumn{2}{c}{} \\ 
  &   &  1     &  2   &   &  \\
\cline{2-5}
  &1  & 0.0   & 1.0 & 1.0 &  \\
S &2  & 0.0   & 1.0 & 1.0 &  \\
  &3  & 1.0   & 0.0 & 1.0 &  \\
\cline{2-5} 
  &   &       &      &     & \\ 
\end{tabular}
\caption{M--step Iteration 2:  $p(S)$ (left), $p(F_1|S)$ (center),
$p(F_2|S)$ (right)} 
\label{fig:mstep2}
\end{center}
\myendfig   

At this point two iterations of the EM algorithm have been performed. 
From this point forward, at the end of each iteration a check for
convergence is performed. The parameters estimated during the previous
iteration are $\Theta^{old}$ and those estimated during the second
iteration are $\Theta^{new}$. For example, from iterations 1 and 2 the
following estimates have been made:
\begin{eqnarray*}
\Theta^{old} = \{.4, .4, .2, .75, .25, .5, .5, 1.0, 0.0, .25, .75, .25, .75,
.5, .5\}  \\
\Theta^{new} = \{.4, .3, .3, 1.0, 0.0, 0.0, 1.0, 1.0, 0.0, 0.0, 1.0, 0.0,
1.0, 1.0, 0.0\} 
\end{eqnarray*}

The differences between $\Theta^{old}$ and $\Theta^{old}$ are
considerable and certainly more than a typical value of $\epsilon$,
i.e., .01 or .001.  Thus, the EM algorithm continues for at least
one more iteration.  

{\bf E--step Iteration 3:}
The values for the marginal event counts are re--estimated by finding the
value of $S$ that maximizes the conditional probability distributions
$p(S|F_1, F_2)$. This calculation is made from the parameter estimates 
found in the M--step   of the previous iteration, shown in Figure 
\ref{fig:mstep2}. 

\begin{figure}
\begin{center}
\begin{tabular}{ccc|c}
$F_1$ & $F_2$ & $S$ & $p(S|F_1,F_2)$ \\  \hline
 1    &   1   &  1  &  0.0  \\
 1    &   1   &  2  &  0.0  \\
 1    &   1   &  3  &  {\bf 1.0}  \\ \hline
 1    &   2   &  1  &  {\bf 1.0}  \\
 1    &   2   &  2  &  0.0  \\
 1    &   2   &  3  &  0.0  \\ \hline
 2    &   1   &  1  &  0.0  \\
 2    &   1   &  2  &  0.0  \\
 2    &   1   &  3  &  0.0  \\  \hline
 2    &   2   &  1  &  0.0  \\
 2    &   2   &  2  &  {\bf 1.0}  \\
 2    &   2   &  3  &  0.0  \\
\end{tabular}
\caption{E--Step Iteration 3}
\label{fig:estep3}
\end{center}
\myendfig   

The probabilities in bold face in Figure \ref{fig:estep3} are the 
maximum for $\hat p(S|F_1,F_2)$, given a particular pair of feature
values  $(f_1,f_2)$. New values for $S$ replace the previous values in
the data sample, as shown in Figure \ref{fig:estep3a}. However, the
values found during the third iteration prove to be identical to those
found during the second iteration. 

\begin{figure}
\begin{center}
\begin{tabular}{cc|c}
$F_1$ & $F_2$ & S \\  \hline
1 & 2 & 1  \\
1 & 2 & 1  \\
2 & 2 & 2  \\
2 & 2 & 2  \\
1 & 2 & 1  \\
1 & 1 & 3  \\
1 & 1 & 3  \\
1 & 1 & 3  \\
1 & 2 & 1  \\
2 & 2 & 2  \\ 
\end{tabular}
\caption{E--Step Iteration 3}
\label{fig:estep3a}
\end{center}
\myendfig   

Both the resulting contingency table representation of the
expected marginal event counts and the resulting parameter estimates
will be identical in iteration 3 to those found in iteration 2. 
Given this, the difference between $\Theta^{old}$ and $\Theta^{new}$ will
be zero and the EM algorithm will converge. Thus the values for the
missing variables $S$ are as shown in Figure \ref{fig:estep3a}. This
appears to be a reasonable result. The feature values $(F_1=1,F_2=1)$
belong to class 3, the feature values $(F_1=2,F_2=2)$ belong to class
2, and the feature values $(F_1=1,F_2=2)$ belong to class 1. 

\end{thesis}

\end{document}


==> junk/gibbs.tex <==
\input{head.tex}
\begin{thesis}

\chapter{Gibbs}

The same example that was used with the EM algorithm is employed here 
to illustrate Gibbs Sampling. The original data sample from the EM
algorithm example is also used here; it is shown in Table \ref{tab:data}. 
Again, assume that the parametric form of the model is Naive Bayes: 
\begin{equation}
\hat p(F_1,F_2,S) = \hat p(S) \times \hat p(F_1|S) \times \hat p(F_2|S)
\end{equation}
where the parameters of the model are $p(S)$, $p(F_1|S)$, and $p(F_2|S)$. 

{\bf Stochastic E--Step Iteration 1}: Like the EM algorithm, Gibbs 
Sampling begins by randomly assigning values to $S$. Assume that the 
random assignment of values to  $S$ and the resulting contingency table
representation of marginal event counts is as shown in Figure 
\ref{fig:gibbe1}. 

\begin{figure}
\begin{center}
\begin{tabular}{cc|ccc}
$F_1$ & $F_2$ & S  & & \\  
\cline{1-3}
1 & 2 & 1 & &  \\
1 & 2 & 3 & &  \\
2 & 2 & 2 & &  \\
2 & 2 & 2 & &  \\
1 & 2 & 1 & &  \\
1 & 1 & 3 & &  \\
1 & 1 & 1 & &  \\
1 & 1 & 2 & &  \\
1 & 2 & 2 & &  \\
2 & 2 & 1 & &  \\ 
\end{tabular}
\begin{tabular}{cc|cc|ccc} 
\multicolumn{2}{c}{} & 
\multicolumn{2}{c}{$F_1$} & 
\multicolumn{3}{c}{} \\
  &   &  1  &  2 & & &   \\ 
\cline{2-5}
  & 1 &  3  &  1 & 4 & &  \\
S & 2 &  2  &  2 & 4 & & \\
  & 3 &  2  &  0 & 2 & & \\
\cline{2-5}
  &   &  7  &  3 & 10 & & \\ 
\end{tabular}
\begin{tabular}{cc|cc|ccc} 
\multicolumn{2}{c}{} & 
\multicolumn{2}{c}{$F_2$} & 
\multicolumn{3}{c}{} \\
  &   &  1  &  2 &  & &   \\ 
\cline{2-5}
  & 1 &  1  &  3 & 4 & &  \\
S & 2 &  1  &  3 & 4 & &  \\
  & 3 &  1  &  1 & 2 & &  \\
\cline{2-5}
  &   &  7  &  3 & 10 & & \\ 
\end{tabular}
\label{fig:gibbe1}
\caption{Stochastic E--Step Iteration 1}
\end{center}
\myendfig   

{\bf Stochastic M---Step Iteration 1}
In the EM algorithm the marginal event counts shown in the contingency
tables in Figure \ref{fig:gibbe1} are used to directly compute maximum 
likelihood estimates for the model parameters. However, in Gibbs Sampling
no maximum likelihood estimates are computed; instead, the marginal event 
counts combine with prior knowledge of the problem to form a
posterior distribution from which values for the model parameters
are sampled. 

Each row in the contingency tables shown in Figure \ref{fig:gibbe1} 
represents a conditional probability distribution that can in turn be 
represented by a multinomial distribution. This observed multinomial will
be multiplied by a Dirichlet prior to define a posterior distribution from
which to sample values for the model. The multinomial distribution is
represented in terms of the observed event counts. For example, given that
S is fixed at 1, $freq(F_1|S=1)$ = $M(3,1)$. Prior distributions are
expressed in much the same way. However, in this example the priors
are non--informative and of the form $D(1,1)$. This shows that there
are two possible events and each was observed 1 time. 

Thus, from Figure \ref{fig:gibbe1} the following sampling scheme is
created, based on the observed multinomial data and the assumption of
non--informative priors:
\begin{eqnarray*}
p(F_1 | S=1) \sim D(4,2) = M(3,1) \times  D(1,1) \\
p(F_1 | S=2) \sim D(3,3) = M(2,2) \times  D(1,1) \\
p(F_1 | S=3) \sim D(3,1) = M(2,0) \times  D(1,1) \\
p(F_2 | S=1) \sim D(2,4) = M(1,3) \times  D(1,1) \\
p(F_2 | S=2) \sim D(2,4) = M(1,3) \times  D(1,1) \\
p(F_2 | S=3) \sim D(2,2) = M(1,1) \times  D(1,1) \\
p(S) \sim D(5,5,3) = M(4,4,2) \times D(1,1,1)  
\end{eqnarray*}

\begin{figure}
\begin{center}
\begin{tabular}{cc|c|ccc} 
  &   &         & & & \\
\cline{2-4}
  & 1 &  0.03    & & &  \\
S & 2 &  0.51    & & & \\
  & 3 &  0.47    & & & \\
\cline{2-4} 
  &   &         & & & \\
\end{tabular}
\begin{tabular}{cc|cc|cccc} 
\multicolumn{2}{c}{} & 
\multicolumn{2}{c}{$F_1$} & 
\multicolumn{4}{c}{} \\ 
  &   &  1     &  2    &      & & & \\
\cline{2-5}
  & 1 &  0.64  &  0.36 & 1.0 & & &  \\
S & 2 &  0.54  &  0.46 & 1.0 & & &  \\
  & 3 &  0.76  &  0.24 & 1.0 & & &  \\
\cline{2-5} 
  &   &        &       &      & & &  \\ 
\end{tabular}
\begin{tabular}{cc|cc|cc} 
\multicolumn{2}{c}{} & 
\multicolumn{2}{c}{$F_2$} & 
\multicolumn{2}{c}{} \\ 
  &   &  1     &  2   &   &  \\
\cline{2-5}
  &1  & 0.37  & 0.63 & 1.0 &  \\
S &2  & 0.09  & 0.91 & 1.0 &  \\
  &3  & 0.73  & 0.27 & 1.0 &  \\
\cline{2-5} 
  &   &       &      &     & \\ 
\end{tabular}
\label{fig:gibbm1}
\caption{Stochastic M--step Iteration 1: 
$\hat p(S)$ (left), $\hat p(F_1|S)$ (center), $\hat p(F_2|S)$ (right)}  
\end{center}
\myendfig   

The parameter estimates shown in Figure \ref{fig:gibbm1} result from 
sampling values from the posterior Dirichlet  distributions defined by
multiplying the observed multinomial data and an uninformative prior
distribution.  

{\bf E--Step Iteration 2}
After the first iteration of Gibbs Sampling, all subsequent
iterations arrive at new values for the marginal event counts by
sampling new values for $S$ based on the following: 

\begin{equation}
S = \stackrel{argmax}{s} p(S | F_1, F_2) = \frac{p(S) \times p(F_1|S)
\times p(F_2|S)}{p(F_1,F_2)} 
\end{equation}

This computation is made using the parameter estimates in Figure
\ref{fig:gibbm1} that were arrived at during the stochastic M--step of the 
previous iteration. The estimates of $p(S|F_1,F_2)$ are computed 
deterministically based on the sampled parameter estimates. The results of
this computation are shown in Figure \ref{fig:gibbe2}. 


\begin{figure}
\begin{center}
\begin{tabular}{ccc|c}
$F_1$ & $F_2$ & $S$ & $p(S|F_1,F_2)$ \\  \hline
 1    &   1   &  1  &  .024  \\
 1    &   1   &  2  &  .085  \\
 1    &   1   &  3  &  .891  \\ \hline
 1    &   2   &  1  &  .033  \\
 1    &   2   &  2  &  .699  \\
 1    &   2   &  3  &  .267 \\ \hline
 2    &   1   &  1  &  .100  \\
 2    &   1   &  2  &  .525  \\
 2    &   1   &  3  &  .375  \\  \hline
 2    &   2   &  1  &  .028  \\
 2    &   2   &  2  &  .852  \\
 2    &   2   &  3  &  .120  \\
\end{tabular}
\label{fig:gibbe2}
\caption{E--Step Iteration 2}
\end{center}
\myendfig   

However, rather than imputing the value of $S$ that maximizes 
$p(S|F_1,F_2)$, as is the case in the EM algorithm, instead values of 
$S$ are sampled, based upon the conditional distributions defined
by $p(S|F_1,F_2)$. The imputed values for $S$, arrived at via sampling,
are shown in Figure \ref{fig:gibbe2a}.  Note that the first two
observations in the data sample have the same observed feature values 
$(F_1=1, F_2=2)$. However, different values of $S$ are imputed 
due to the fact that the imputed values result from a sampling rather
than maximization operation. 

\begin{figure}
\begin{center}
\begin{tabular}{cc|ccc}
$F_1$ & $F_2$ & S \\  
\cline{1-3}
1 & 2 & 2 & &  \\
1 & 2 & 3 & &  \\
2 & 2 & 2 & &  \\
2 & 2 & 2 & &  \\
1 & 2 & 3 & &  \\
1 & 1 & 3 & &  \\
1 & 1 & 3 & &  \\
1 & 1 & 3 & &  \\
1 & 2 & 2 & &  \\
2 & 2 & 2 & &  \\ 
\end{tabular}
\begin{tabular}{cc|cc|ccc} 
\multicolumn{2}{c}{} & 
\multicolumn{2}{c}{$F_1$} & 
\multicolumn{3}{c}{} \\
  &   &  1  &  2 &  & &   \\ 
\cline{2-5}
  & 1 &  0  &  0 & 0 & &  \\
S & 2 &  2  &  3 & 5 & &  \\
  & 3 &  5  &  0 & 5 & &  \\
\cline{2-5}
  &   &  7  &  3 & 10 & & \\ 
\end{tabular}
\begin{tabular}{cc|cc|ccc} 
\multicolumn{2}{c}{} & 
\multicolumn{2}{c}{$F_2$} & 
\multicolumn{3}{c}{} \\
  &   &  1  &  2 &  & &   \\ 
\cline{2-5}
  & 1 &  0  &  0 & 0 & &  \\
S & 2 &  0  &  5 & 5 & &  \\
  & 3 &  3  &  2 & 5 & &  \\
\cline{2-5}
  &   &  3  &  7 & 10 & &  \\ 
\end{tabular}
\caption{Stochastic E--Step Iteration 2}
\label{fig:gibbe2a}
\end{center}
\myendfig   

Figure \ref{fig:gibbe2a} also shows the contingency tables that result
from the imputed values of $S$. 

{\bf M--Step Iteration 2}
Given the marginal event counts found during the stochastic E--step, 
sampling from the Dirichlet posterior of the model parameters is performed  
according to the following scheme: 

\begin{eqnarray*}
p(F_1|S=1) \sim D(1,1) =  M(0,0) + D(1,1) \\
p(F_1|S=2) \sim D(3,4) =  M(2,3) + D(1,1) \\
p(F_1|S=3) \sim D(6,1) =  M(5,0) + D(1,1) \\
p(F_2|S=1) \sim D(1,1) =  M(0,0) + D(1,1) \\
p(F_2|S=2) \sim D(1,6) =  M(0,5) + D(1,1) \\
p(F_2|S=3) \sim D(4,3) =  M(3,2) + D(1,1) \\
p(S) \sim D(1,6,6) =  M(0,5,5) + D(1,1,1) 
\end{eqnarray*}

Figure \ref{fig:gibbm2} shows the sampled estimates for $p(S)$, 
$p(F_1|S)$, and,  $p(F_2|S)$. 

\begin{figure}
\begin{center}
\begin{tabular}{cc|c|ccc} 
  &   &         & & & \\
\cline{2-4}
  & 1 &  0.06    & & &  \\
S & 2 &  0.54    & & & \\
  & 3 &  0.40    & & & \\
\cline{2-4} 
  &   &         & & & \\ 
\end{tabular}
\begin{tabular}{cc|cc|cccc} 
\multicolumn{2}{c}{} & 
\multicolumn{2}{c}{$F_1$} & 
\multicolumn{4}{c}{} \\ 
  &   &  1     &  2    &      & & & \\
\cline{2-5}
  & 1 &  0.25  &  0.75 & 1.0 & & &  \\
S & 2 &  0.68  &  0.32 & 1.0 & & &  \\
  & 3 &  0.93  &  0.06 & 1.0 & & &  \\
\cline{2-5} 
  &   &        &       &   & & &  \\ 
\end{tabular}
\begin{tabular}{cc|cc|cc} 
\multicolumn{2}{c}{} & 
\multicolumn{2}{c}{$F_2$} & 
\multicolumn{2}{c}{} \\ 
  &   &  1     &  2   &   &  \\
\cline{2-5}
  &1  & 0.16   & 0.84 & 1.0 &  \\
S &2  & 0.05   & 0.95 & 1.0 &  \\
  &3  & 0.52   & 0.48 & 1.0 &  \\
\cline{2-5} 
  &   &       &      &     & \\ 
\end{tabular}
\label{fig:gibbm2}
\caption{Stochastic M--step Iteration 2:  
$\hat p(S)$ (left), $\hat p(F_1|S)$ (center), $\hat p(F_2|S)$ (right)} 
\end{center}
\myendfig   

The sampling of these estimates concludes the stochastic M--step and the 
second iteration of Gibbs Sampling has concluded. 

{\bf Stochastic E--step Iteration 3}
Given the parameter estimates from the previous stochastic M--step,
shown in Figure \ref{fig:gibbm2}, a new distribution of $S$ is computed 
using those estimates:

\begin{equation}
S = \stackrel{argmax}{s} p(S | F_1, F_2) = \frac{p(S) \times p(F_1|S)
\times p(F_2|S)}{p(F_1,F_2)} 
\end{equation}

The results of this computation are shown in Figure \ref{fig:gibbe3},
which defines the conditional distributions $p(S|F_1, F_2)$. 

\begin{figure}
\begin{center}
\begin{tabular}{ccc|c}
$F_1$ & $F_2$ & $S$ & $p(S|F_1,F_2)$ \\  \hline
 1    &   1   &  1  &  0.009  \\
 1    &   1   &  2  &  0.085  \\
 1    &   1   &  3  &  0.906  \\ \hline
 1    &   2   &  1  &  0.024  \\
 1    &   2   &  2  &  0.645  \\
 1    &   2   &  3  &  0.331  \\ \hline
 2    &   1   &  1  &  0.250  \\
 2    &   1   &  2  &  0.321  \\
 2    &   1   &  3  &  0.429  \\  \hline
 2    &   2   &  1  &  0.181  \\
 2    &   2   &  2  &  0.759  \\
 2    &   2   &  3  &  0.056  \\
\end{tabular}
\label{fig:gibbe3}
\caption{Stochastic E--Step Iteration 3}
\end{center}
\myendfig   

From those distributions new imputed values for $S$ are sampled. The
results of this sampling operation are shown in Figure \ref{fig:gibbe3a}. 

\begin{figure}
\begin{center}
\begin{tabular}{cc|c}
$F_1$ & $F_2$ & S \\  \hline
1 & 2 & 2  \\
1 & 2 & 2  \\
2 & 2 & 2  \\
2 & 2 & 2  \\
1 & 2 & 3  \\
1 & 1 & 3  \\
1 & 1 & 3  \\
1 & 1 & 3  \\
1 & 2 & 2  \\
2 & 2 & 2  \\ 
\end{tabular}
\label{fig:gibbe3a}
\caption{Stochastic E--Step Iteration 3}
\end{center}
\myendfig   

Again, the resulting contingency tables are formed and are used to define
the multinomial distribution that will be used to create the posterior
distribution from which to sample new estimates for the model parameters. 

Normally Gibbs Sampling continues for hundreds of iterations. However, for 
the sake of this demonstration no further calculations or sampling
operations will be shown, instead a few points about monitoring 
convergence  will be made at this point. A chain of values is made for 
each imputed value of $S$ and for each parameter estimate. Each chain is 
monitored for convergence using Geweke's measure \cite{Geweke92}.  

In Geweke's method, a chain is divided into two windows, where one
window occurs at the beginning of the chain and the other occurs at
the end of the chain. Here each window consists of about 10 \% of the
total number of iterations in the chain. If the entire chain has reached a
stationary distribution, then these two windows, one early in the chain
and the other late,  should have approximately the same mean values. 
\end{thesis}

\end{document}


==> junk/single.tex <==

\input{head.tex}

\begin{thesis}

\input{chap1.tex}  %   1. Introduction  (done, ?)

%\input{chap2.tex}   %  2. Background (done, ok)
 
%\input{chap3.tex}   %  3. Supervised Learning (done, ?)

%\input{chap4.tex}   %  4. Unsupervised Learning (done, ?)

%\input{chap5.tex}   %  5. Experimental Data (done, ok)

%\input{chap6.tex}   %  6. Supervised Experimental Results (done, ok)

%\input{chap7.tex}   %  7. Unsupervised Experimental Results (done, ok)

\input{chap8.tex}   %  8. Related Work

%\input{chap9.tex}   %  9. Conclusion


% ******************  bibliography  ******************  

%\bibliographystyle{/users/research/rbruce/group/papers/sty/fullname}
%\bibliography{/users/research/rbruce/group/papers/bib/tdp}

%\bibliographystyle{acm}
%\bibliography{/users/research/rbruce/group/papers/bib/tdp}

\end{thesis}
 
\end{document}

